A depleted and numerical model for pulsed Gaussian wave type II second harmonic generation

This paper presents a three-dimensional (3-D) and spatio-temporal dependent nonlinear wave model to explain the generation of pulsed Gaussian Second Harmonic Waves (SHW). We solve numerically three coupled equations describing the type II Second Harmonic Generation (SHG) in cylindrical KTP crystals under the assumption of fundamental waves depletion, two for ordinary and one for extraordinary Fundamental Waves (FW). The results are attained by a homemade code written in FORTRAN. The results depict the efficiency of the SHG process with the conversion of FW energy to SHW energy, while SHW keeps the same Gaussian profile as FW. Furthermore, the results examine the effect of pulse energy, beam spot size, and therefore interaction length on SHW efficiency.

==> tex/latexmkrc.tex <==
$ENV{'TEXINPUTS'}='./tex//:' . $ENV{'TEXINPUTS'}; 
$ENV{'BSTINPUTS'}='./bst//:' . $ENV{'BSTINPUTS'};
